Marked Neural Spatio-Temporal Point Process Involving a Dynamic Graph Neural Network

Temporal Point Processes (TPPs) have recently become increasingly interesting for learning dynamics in graph data. A reason for this is that learning on dynamic graph data is becoming more relevant, since data from many scientific fields, ranging from mathematics, biology, social sciences, and physics to computer science, is naturally related and inherently dynamic. In addition, TPPs provide a meaningful characterization of event streams and a prediction mechanism for future events. Therefore, (semi-)parameterized Neural TPPs have been introduced whose characterization can be (partially) learned and, thus, enable the representation of more complex phenomena. However, the research on modeling dynamic graphs with TPPs is relatively young, and only a few models for node attribute changes or evolving edges have been proposed yet. To allow for learning on fully dynamic graph streams, i.e., graphs that can change in their structure (addition/deletion of nodes/edge) and in their node/edge attributes, we propose a Marked Neural Spatio-Temporal Point Process (MNSTPP). It leverages a Dynamic Graph Neural Network to learn a Marked TPP that handles attributes and spatial data to model and predict any event in a graph stream.

==> Experiments/baselines.tex <==
\subsection{Baseline Models}

\begin{table}[h!]
    \hspace{-3cm}
    \begin{tabular}{c|c|c|c|c}
        Name+Ref & Task & Note & Code Link & RW-DS \\
        \hline
         NHP-mei & event type, time pred & TPP general (non-graph) & \href{https://github.com/hongyuanmei/neurawkes}{GitHub} &\multirow{7}{*}{\href{https://meta.wikimedia.org/wiki/Data_dumps}{Wikipedia}, \href{http://files.pushshift.io/reddit/}{Reddit}\footnotemark, MOOC}\\
         DyREP \cite{inproc_trivedi_2019} & link, time pred\footnotemark  & TPP based (edge-evolv) & \href{https://github.com/Harryi0/dyrep_torch/tree/main/Synthetic}{GitHub}& \\
         GHNN\cite{han2020graph} & link \& time pred & KG, TPP (edge-evolv)& \href{https://github.com/Jeff20100601/GHNN_clean}{Github}& \\
         \href{https://www.mdpi.com/2504-4990/5/4/69}{GTHP-GNN} & dyn link pred & Hawkes NTPP snapshots & ?? &\\\cline{1-4} %\href{https://snap.stanford.edu/data/Oregon-2.html}{AS-Oregon-2},\href{https://snap.stanford.edu/data/as-733.html}{AS-733}
         $TGN_{attn}$ \cite{arx_rossi_2020} & link pred, node classification\footnotemark & msg pass/fully dyn CTDR & \href{https://paperswithcode.com/paper/temporal-graph-networks-for-deep-learning-on#code}{Paper with Code} & \\ 
         % TGAT\cite{TGAT} & link pred, node classification & which graph type? &\href{https://paperswithcode.com/paper/inductive-representation-learning-on-temporal-1}{Paper with Code}& \href{http://snap.stanford.edu/jodie/wikipedia.csv}{Wikipedoa}, \href{http://snap.stanford.edu/jodie/reddit.csv}{Reddit}, \href{https://grocery.walmart.com/}{Walmart}\\ 
         PINT\cite{PINT} & dyn link pred & TGN+PE, fully dyn CTDR & \href{https://github.com/AaltoPML/PINT/tree/main}{Original Code} & \\
         CAW\cite{CAW} & dyn link pred & RNN, edge-evolv & \href{http://snap.stanford.edu/caw/}{Project},\href{https://github.com/snap-stanford/CAW}{Code} & \\\hline\hline
         %NAT \cite{NAT} & link pred & & \href{https://paperswithcode.com/paper/neighborhood-aware-scalable-temporal-network}{Paper with Code}&\\ \hline
         %StemGNN & multivar ts pred & g struct static, SShot & \href{https://paperswithcode.com/paper/spectral-temporal-graph-neural-network-for-1}{Papers with Code} & 9 different datasets\\ 
         %\href{https://dl.acm.org/doi/abs/10.1145/3366423.3380186}{STPP} & ts pred & snapshots & \href{https://github.com/LMissher/STGNN}{Original code?}& traffic (METR-LA , PEMS-BAY)\\ 
         \href{https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9146162}{STGAT} & ts prediction traffic & & \href{https://github.com/xyk0058/STGAT}{original?} \href{https://github.com/SakastLord/STGAT}{or this?}& \multirow{3}{*}{METR-LA , PEMS-BAY}\\ 
         \href{https://dl.acm.org/doi/pdf/10.1145/3532611}{DGCRN} & & & \href{https://github.com/tsinghua-fib-lab/Traffic-Benchmark}{code} & \\
         \href{https://dl.acm.org/doi/pdf/10.1145/3394486.3403118?casa_token=fqMb36bC5RUAAAAA:ZJtF6JM8jT5JsrAS49TnD3R3qTU5S-DO3WdVBr5dAV_N2z9e6XxuRsGXifW1sxCYZDbms_ppgasS****}{MTGNN} & & ist im benchmark oben drin & & \\
         %\href{https://dl.acm.org/doi/abs/10.1145/3534678.3539396}{STEP} & & & \href{https://github.com/zezhishao/STEP}{official code}&  METR-LA, PEMS-BAY, PEMS04  \\ 
         %\href{https://proceedings.mlr.press/v162/lan22a/lan22a.pdf}{DSTAGNN} & & & \href{https://github.com/SYLan2019/DSTAGNN}{code}& PEMS03, 04, 07, 08 \\
         %\href{https://www.ijcai.org/proceedings/2018/0505.pdf}{\textbf{STGCN}} & &jeder nimmt das & \href{https://github.com/VeritasYin/STGCN_IJCAI-18}{code} & ganz andere \\ 
         %\href{https://arxiv.org/pdf/2206.09112}{D2STGNN} & & decouplen was & \href{https://github.com/zezhishao/D2STGNN}{official code}& METR-LA, PEMS-BAY, PEMS 04,08\\ \hline
         %Masttertyp & time, attribute pred & S are $R^2$ coordinates & \href{https://proceedings.mlr.press/v168/zhou22a.html}{wo code?}& \\
          %& & & \href{https://openreview.net/pdf?id=ESVGfJM9a7}{hier mit appendix} &\\
          %& & & \href{https://escholarship.org/uc/item/3sn484cn#page=57}{hier die thesis} &\\
          %& & & \href{https://github.com/Rose-STL-Lab/DeepSTPP}{Code gefunden} &\\
          %DynGEM & link pred (nur embed gelernt) & & \href{https://github.com/palash1992/DynamicGEM}{GitHub} & komplett andere scheiße\\
          %GAT\cite{GAT} & & & & \\
          %GraphSAGE & node/ graph classification & static graphs? & \href{https://paperswithcode.com/paper/inductive-representation-learning-on-large#code}{Paper with Code}& \href{http://snap.stanford.edu/graphsage/}{Citation, Reddit, Protein}\\ \hline
         
    \end{tabular}
    \caption{Baseline models and the addressed learning tasks.}
    \label{tab:baselines}
\end{table}
\footnotetext[5]{They also compare the embeddings}
\footnotetext[6]{from JODIE model}
\footnotetext[7]{same datasets as in \cite{arx_rossi_2020}, so the JODIE datasets}


Tasks:
\begin{itemize}
    \item Link Prediction: RR@k, $k=10$ (one hit from the first k)
    \item Deletion of nodes and edges (ranking of existing nodes/edges): RR@k, P@k
    \item Event Time Prediction: RMSE, MAE, MAPE
    \item \textbf{Attribute Prediction}: RMSE, MAE, MAPE
    \item event type prediction: F1-score
\medskip


    
\end{itemize}

Baseline modelle genutzt bei den TPPs:
\begin{itemize}
    \item Intensity RNN (Modeling the intensity function of point process via recurrent neural networks)
    \item Recurrent Marked Temporal Point Process (Recurrent marked temporal point processes: Embedding event history to vector)
    \item Neural Hawkes Process (The neural Hawkes process: A neurally self-modulating multivariate point process)
    \item Astrologer 
\end{itemize}

==> Experiments/datasets.tex <==
\subsection{Datasets}
\subsubsection{Synthetic Datasets}

\subsubsection{Real-World Datasets}
\paragraph{MOOC Activity Dataset.} For learning structural dynamics (addition and deletions of nodes and edges) in a graph stream, we utilize the MOOC activity dataset taken from \cite{MOOC_data}. The MOOC platform (Massive Open Online Courses\footnote{\url{https://www.mooc.org/}}) provides several free online courses from different domains and the dataset consists of an activity event stream of users on the platform. It contains 411,749 timestamped interactions of 7,047 users with 98 online courses and 4,066 drop-out events (=0.98\%) where users drop out of a course after an interaction. The raw dataset includes an activity stream of user-course pairs with timestamp, 4-dimensional attribute and a label, whether the user dropped out or not. For the experiments in this paper, the stream has been modified to match the form of events as tuples $($item, time, event type, attribute$)$ and thus contains 680,213 events of additions and deletions of nodes and edges in total. The number of events increased, because we added the node addition events before an edge has been added and node deletion, if the last incident edge has been deleted. In addition, if there is a duplicate addition or deletion of a node or edge it as been artificially deleted or added beforehand.


\paragraph{METR-LA, PEMS-BAY.} 
We utilize traffic network datasets to capture attribute dynamic data,  drawing upon widely used sources such as METR-LA and PEMS-BAY used in \cite{DCRNN}.
These datasets provide insights into the behavior of traffic networks, giving information on variables such as traffic flow, speed, and occupancy. METR-LA encompasses traffic data collected from loop detectors deployed on the freeways in Los Angeles, capturing the real-time traffic conditions across various city regions. Similarly, PEMS-BAY consists of traffic data collected from the Bay Area in California.
The given data is preprocessed as follows:
First, the provided weighted adjacency matrix is used to construct a directed graph, where each edge has this weight as an attribute. 
Additionally, self-loops are removed. Then, the node attributes from the first timestamp are taken as attributes for the initial graph, with all subsequent attributes representing node attribute change events happening every 5 minutes. 
For each node, one event is generated. Events where the attribute has not changed since the last timestamp are filtered out to prevent the graph from becoming too large.

==> Experiments/evaluation.tex <==
\subsection{Evaluation}
\begin{itemize}
    \item train, validation, test set split $70-15-15\%$ \cite{TGAT}
    \item prediction on validation and test set
    \item prediction of time and attribute is regression, so we use most commonly used metrics: RMSE, MAE, MAPE \\
    Mean Absolute Error (MAE),
Root Mean Squared Error (RMSE) and Mean Absolute Percentage
Error (MAPE). The formulas are as follows:
\begin{align}
    \text{MAE}(\mathbf{x}, \hat{\mathbf{x}}) &= \frac{1}{|\Omega|} \sum_{i \in \Omega} |\mathbf{x}_i - \hat{\mathbf{x}}_i| \\
    \text{RMSE}(\mathbf{x}, \hat{\mathbf{x}}) &= \sqrt{\frac{1}{|\Omega|} \sum_{i \in \Omega} (\mathbf{x}_i - \hat{\mathbf{x}}_i)^2} \\
    \text{MAPE}(\mathbf{x}, \hat{\mathbf{x}}) &= \frac{1}{|\Omega|} \sum_{i \in \Omega} \left| \frac{\mathbf{x}_i - \hat{\mathbf{x}}_i}{\mathbf{x}_i} \right|,
\end{align}
where MAE metric reflects the prediction accuracy, RMSE is more sensitive to abnormal values, and MAPE can somewhat eliminate the influence of data units. $\mathbf{x}_i$ denotes the $i$-th ground truth, $\hat{\mathbf{x}}_i$ represents the $i$-th predicted value, and $\Omega$ is the set of indices of observed samples, where $|\Omega| = T_f = 12$ in our experiments. \textcolor{red}{Anpassen auf under paper.}
    \item event type prediction is multiclass-classification, so we use BCELoss for multiclass
    \item node/edge prediction is evaluated by ranking, so MRR, HIT@k,...
\end{itemize} 

==> Experiments/experimental_setup.tex <==
\subsection{Experimental Setup}

We use:
\begin{itemize}
    \item biases in all layers
    \item batching analoguously to the dependency-graph-driven event parallelization from \cite{chen2023neutronstream}
    \item standardized attributes
    \item logarithmic-scaled timestamps
\end{itemize}

Comments for reproducability:
\begin{itemize}
    \item the radii of the open ball and the time interval in the predictions are $\varepsilon=\Delta \tau = 10^{-7}$ (the second double integral for the event probability)
    \item while the double integrals for the predictions are not evaluated on $[\bar{t},\infty]$ and $\mathbb{R}^d$, but due to the logarithmic scale of the time and the standardization of the attributes (each dimension separately) the integrals are approximated over $\tau \in [\text{log}\,(\bar{t}), \text{log}\,(\bar{t}+2\cdot \text{max}(\Delta t)))$ and $\bm{\delta}\in [-3,3]^d$ (the decision of $3$ comes from $3$-times the standard deviation of $1$ to include $99.9\%$ of the observed data)
    \item the negative samples' attributes are sampled from a fixed ball around an existing attribute, while their timestamps are in an interval around a given timestamp with a length dependent on the timestamp, as e.g., $[t-.1\cdot t,t+.1\cdot t]$
\end{itemize}

==> other_sections/discussion.tex <==
\section{Discussion}

\textcolor{red}{How to predict in \textit{inductive} and \textit{transductive} manner?}

==> preliminaries_subsections/DGNN.tex <==
\subsection{Dynamic Graph Neural Network}

==> preliminaries_subsections/tpps1.tex <==
\subsection{Temporal Point Processes}
%A sequence of observations can be regarded as a random process. Each event at a point in time is then treated as a random variable, which in turn depends on the previous observations. This is referred to as a Temporal Point Process (TPP). Temporal Point Processes provide a conditional density function that acts as a function over time and comes with an approach to predict new events in the future. 
A sequence of observations forms a temporal point process (TPP), where each event at a given time point is treated as a random variable influenced by previous observations. TPPs offer a conditional density function that operates over time, enabling the prediction of future events.
%can be characterized as a counting function quantifying the number of events occuring at points in time. 
%The model proposed here is a specific TPP, a \textbf{Marked Neural Spatio-Temporal Point Process (MNSTPP)}, to utilize these advantages. It enables processing event streams including attributed and spatial events in a graph without prior knowledge about the temporal behavior of the stream. In the following, the Marked and Spatio-Temporal Point Process are defined for attributed (marked) and spatial events. Afterwards, the concept of Neural Temporal Point Processes is introduced that relieves the assumptions of specific temporal patterns in the process and enables the learning of the temporal evolution of an input stream.
The proposed model is a specialized type of temporal point process known as a \textbf{Marked Neural Spatio-Temporal Point Process (MNSTPP)}. It capitalizes on these benefits by handling event streams comprising attributed and spatial events within a graph without requiring prior knowledge about the temporal dynamics of the stream.
Firstly, the definitions of Marked and Spatio-Temporal Point Processes are presented for attributed and spatial events, respectively. Subsequently, the concept of Neural Temporal Point Processes is introduced, which relaxes assumptions about specific temporal patterns in the process and enables learning the temporal evolution of an input stream.

\begin{paragraph}{Marked Temporal Point Processes.}
Given an event stream, it is non-trivial to tell when a new event will occur and what it may look like. Given that the event is dependent on the historical point patterns, the underlying process can be modeled as a \textbf{Temporal Point Process (TPP)} \cite{TPP_lecture}. Furthermore, the events in a graph stream as defined above include the timestamps together with additional information as the item, the event type and an attribute. Consequently, the process is modeled as a \textbf{Marked TPP (MTPP)}, where the marks $\bm{m}$ in the following comprise the additional information, so $\bm{m} =(x,k,\gamma_t(x))$. As a result, the marks can be discrete, continuous or a combination of both. Here, the marks in the MTPP are assumed to be i.i.d., i.e., a mark is only dependent on the timestamp but independent from its surrounding in space.

\begin{NDef}[Marked Temporal Point Process]
Let $\set{H}=\{(t_i, \bm{m}_i)\}_{i\in[n]_0}$ be a sequence of $n> 0$ events with marks $\bm{m}_i\in\mathcal{M}$ in space $\mathcal{M}$ and timestamps $t_i\geq 0$. Further, let ${\set{H}_{\bar{t}}=\{(t_i, \bm{m}_i)\mid t_i\leq\bar{t},\ (t_i, \bm{m}_i)\in \set{H}\}}$ entail the history of events before timestamp $t$ up to time $\bar{t}<t$.
Then, the \textbf{conditional intensity} for a new event $(t^*,\bm{m}^*)$ to fall into $[t, t+\Delta t)\times\set{B}(\bm{m})$ given the history is given by
\begin{align}\label{eq_MTPP}
    \lambda(t, \bm{m}\mid \set{H}_{\bar{t}}) = \mathbb{P}\Bigl(t^*\in [t, t+\Delta t), \bm{m}^*\in \set{B}(\bm{m})\mid \set{H}_{\bar{t}}\Bigr)\cdot\mathbb{P}\Bigl(t^*\notin (-\infty,t)\mid \set{H}_{\bar{t}}\Bigr)
\end{align}
and characterizes the MTPP completely \cite{TPP_lecture}. Here, $\set{B}(\bm{m})\subset\mathbb{R}^d$ is an open hypersphere with center $\bm{m}$ and radius $\Delta \bm{m}$ for continuous marks and $\set{B}(\bm{m})=\bm{m}$ for discrete marks. Note that, if $\bm{m}$ is a combination of discrete and continuous marks, then $\set{B}(\bm{m})$ and $\Delta \bm{m}$ are defined component-wise.  
\end{NDef}
The intensity $\lambda$ is determined by the probability of the event to fall into a given ball in the attribute space and time, together with the probability that the event did not happen before (independent whether the attribute already appeared or not). %Fig.~\ref{fig:mtpp} illustrates the probability of an event to fall into a time and attribute interval.
% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=.5\linewidth]{figures/mtpp.png}
%     \caption{The figure is inspired by \cite{STPP_book}. The shaded rectangle is the ball for which we want to have the probability and the dots over time visualize the observed events.}
%     \label{fig:mtpp}
% \end{figure}

According to Campbell's theorem \cite{STPP_book}, the intensity $\lambda$ of an event $(t,x,k,\gamma)$ can also be determined by the expectation of a \textbf{counting function} of $\set{H}$ over the compact set $[t,\Delta t)\times\set{B}(\bm{m})$ as follows:
\begin{align}
    \lambda(t,x,k,\gamma) = \mathbb{E}\bigl[N\bigl([t,\Delta t),\set{B}(\bm{m})\bigr)\bigr] \text{ with}\\
    N([t,\Delta t),\set{B}(\bm{m})) = \sum\limits_{i\in [n]}\mathds{1}_{[t,\Delta t)}(t_i)\cdot\mathds{1}_{\set{B}(\bm{m})}(\bm{m}_i).
\end{align}
The counting function evaluates how often an event of the MTPP falls into the given set using the indicator functions $\mathds{1}$. Since we assume that no two events occur at the same time, the probability of an event is consequently given by
\begin{align}
    \mathbb{P}\Bigl(t_i\in [t, t+\Delta t), \bm{m}_i\in \set{B}(\bm{m})\mid \set{H}_{\bar{t}}\Bigr) = \underset{\Delta m \downarrow \mathds{0}, \Delta t \downarrow 0}{\text{lim}}\frac{\mathbb{E}\bigl[N\bigl([t,\Delta t),\set{B}(\bm{m})\bigr)\bigr]}{|\set{B}(\bm{m})|*\Delta t}.
\end{align}


% \textcolor{red}{Nach Campbell's theorem, gilt dass die intensity $\lambda$ gleich ist mit dem Erwartungswert der Zählfunktion, als $\lambda(t,\bm{m}\mid \set{H}_{\bar{t}}) = \mathbb{E}(N(t))$. Dh aber auch, dass die \textit{wahrscheinlichkeit}, dass ein Event in $B(m,\Delta m),[t,t+\Delta t]$ liegt gegeben ist durch den Erwartungswert geteilt durch das Volumen der Kugel und Zeitinterval $\text{lim}_{\Delta m \downarrow 0, \Delta t \downarrow 0}\frac{\mathbb{E}(N(t))}{|B(m,\Delta m)|*\Delta t}$. }
% \textcolor{red}{Since we assume that no two events occur at the same time, the expectation is equal to the probability of an event to occur in a certain time interval, i.e., $\mathbb{P}(t_i\in[t,t+\Delta t]\mid \set{H}_{\bar{t}})=\mathbb{E}(N([t,t+\Delta t]]))$}

Since the intensity function represents the instantaneous event rate, reflecting the likelihood of an event to occur at a specific time with a specific mark given the historical context, the intensity function must remain non-negative.  
%This function defines the conditional density for an event $o_i$ to occur within the time interval $[t, \Delta t)$ given the historical context, as illustrated in Fig.~\ref{fig:tpp}.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=.5\linewidth]{figures/TPPs.png}
%     \caption{\textcolor{red}{TBD: neu machen mit Referenz zu \cite{TPP}.}}
%     \label{fig:tpp}
% \end{figure}

%Assuming that no events can occur simultaneously, the marked conditional intensity function for \textbf{discrete events} $\bm{m}\in\mathbb{N}$ (such as addition/deletion of nodes/edges in \ref{tab:events}) can be heuristically interpreted as the expectation whether an event occurs at a timestamp given the historical information or not, or as the expected change in case of \textbf{continuous events} $\bm{m}\in\mathbb{R}^d$. 

\begin{NRem}[Spatio-Temporal Point Process]
If the marks of the events $\bm{m}$ determine a location, such as a point in $\mathbb{R}^d$ or a node in a graph, the \textit{Spatio}-Temporal Point Process describes the evolution of data in space and time \cite{STPP}.
\end{NRem}
\end{paragraph}

\begin{paragraph}{Neural Temporal Point Processes.}
%The intensity function of a Point Process has to be chosen carefully based on assumptions about the appearance of temporal patterns in the data. Since these assumptions are not necessarily met in real-world data, partially and fully trainable Neural TPPs \cite{MultiStreamMPP} have been proposed \cite{First_NTPP, NeuralHawkes} to learn the more complex temporal pattern in the data. In the proposed work, we utilize a \textit{partially trainable Neural TPP}, so the definition of the fully-trainable Neural TPP is skipped here but can be found in \cite{MultiStreamMPP}.
The choice of the intensity function in point processes requires careful consideration, typically based on assumptions about the temporal patterns present in the data. However, real-world data often deviates from these assumptions. 
To address this challenge, partially and fully trainable (semi-)parameterized Neural TPPs have been introduced in the literature \cite{First_NTPP, MultiStreamMPP, NeuralHawkes}.
Here, we leverage a semi-parameterized Neural TPP. While the detailed definition of a fully parameterized Neural TPP is omitted here, it can be found in \cite{MultiStreamMPP}.

\begin{NDef}[Neural Temporal Point Process]
Semi-parameterized Neural TPPs \cite{MultiStreamMPP} replace intensity functions by Deep Neural Networks (DNNs). These encode the historical information $\set{H}_{t}$ of an MTPP in a feature vector $\set{H}_{t}$ which is then forwarded to a selected temporal decay function $\phi$. Together, they determine the intensity 
\begin{align}\label{eq_NTPP}
    \lambda(t, \bm{m}\mid \set{H}_{t}) & = \phi(\Delta t, \Delta \bm{m}\mid \set{H}_{t}) %\nonumber
     =\phi(\Delta t, \Delta \bm{m}\mid \text{\textnormal{DNN}}(\set{H}_{t})).
\end{align}
Here, $\Delta t = t - \bar{t}$ and $\Delta \bm{m} = \|\bm{m} - \bar{\bm{m}}\|$ are the deviations of the timestamps and marks from the events at $t$ and the last event before it.
\end{NDef}
\end{paragraph}



